Discovery-Driven Integration of Disjoint Tables via Text

Integrating heterogeneous datasets within data lakes is a critical challenge, particularly for semantically related tables that lack the explicit attributes needed to be joined. We study Discovery-Driven Integration, where the relevant sources and their missing relational structure must be discovered before integration. In this setting, unstructured text provides the evidence that connects otherwise disjoint tables. The fundamental challenge is to discover the relationships at a fine-grained level that connect individual rows from different tables through specific sentences. We formalize this task as Text-Mediated Join Path Discovery and propose a horizontal bidirectional cross-attention architecture called LOKI Latent-space Optimization for Knowledge Integration) that learns contextualized representations of table rows and sentences. Through a global table-text contrastive objective, fine-grained row-sentence associations emerge without explicit local supervision. Existing multi-modal discovery methods largely retrieve coarse-grained column-text associations, whereas integration systems assume supplied row-text links, schemas, or queries. LOKI instead transforms these implicit associations into explicit, interpretable join paths, organizes them into relation-consistent groups, and materializes them as typed integrated tables with sentence-level provenance. Comprehensive evaluations on real-world benchmarks demonstrate that LOKI consistently outperforms state-of-the-art multi-modal data discovery approaches, and materializes typed integrated tables with 0.982 macro typed-pair precision while being up to 40 times cheaper in LLM API cost than direct prompting.

==> old_architecture.tex <==
\section{Architecture of LOKI}

This section details the architecture of \textbf{LOKI}, our proposed solution for the novel problem of \textbf{Discovery-Driven Integration}. We introduce a new paradigm for data integration where unstructured text serves as a semantic bridge between disjoint tables. At its core, LOKI is a new \textbf{multi-modal representation learning architecture} designed to jointly embed structured tabular data and unstructured text into a unified semantic space. The architecture is founded on a \textbf{hierarchical bidirectional cross-attention mechanism} that learns fine-grained, contextualized representations for individual table rows and sentences. A key contribution of our work is that LOKI learns these powerful cross-modal alignments in an entirely self-supervised manner. By training on a coarse-grained, table-document retrieval task, LOKI develops the capability to produce a pair-score matrix without explicit row-sentence supervision (hence hierarchical). From this matrix, we can directly extract \textbf{explicit and interpretable join paths}, a feature that distinguishes LOKI from black-box embedding models. This process allows LOKI to materialize conceptual relationships between tables, even when no explicit join keys exist, without relying on costly, fine-grained annotations.

LOKI's pipeline (see Fig. \ref{fig:pipeline_loki}) is organized into \textbf{six main stages}: \textbf{(1) Input Linearization and Embeddings}, where tables and text are converted into a common format; \textbf{(2) Bidirectional Contextualization}, where the core attention mechanism enriches the representations of each modality with information from the other; \textbf{(3) Scoring and Aggregation}, where both local and global similarity scores are computed; \textbf{(4) Self-Supervised Learning Objective}, which guides the model's training via a multi-task loss function; \textbf{(5) Join Path Extraction}, where high-confidence atomic links are identified and chained through shared mediating sentences; and \textbf{(6) Semantic Materialization}, where join paths are clustered and generalized to derive integrated tables and relational schemas.

\subsection{Stage 1: Input Linearization and Embeddings}

A foundational challenge in cross-modal learning is the representation of disparate data types in a common format. LOKI’s pipeline begins by encoding both structured rows and unstructured sentences into a sequence of embedding vectors. These vectors serve as the primary inputs for the subsequent bidirectional cross-attention mechanism, which is specifically designed to capture and model the complex dependencies between the tabular and textual modalities.

\stitle{1. Row Linearization:} Each row $r_i$ from table $T$ is first transformed into a natural language string. This linearization process concatenates the column names and their cell values for that row:
\begin{equation*}
\operatorname{linearize}(T) = \left[ \text{``}c_1\text{: }v_{i1};\; c_2\text{: }v_{i2};\;\cdots;\; c_{|\mathcal{S}|}\text{: }v_{i|\mathcal{S}|}\text{''} \right]_{i=1}^n \in \mathbb{R}^n
\end{equation*}
For instance, the first row of the \ex{\textit{Patients}} table \ex{$T_1$} in our motivating example would be serialized into the string: ``\ex{\textit{PatientID: $I_1$; Name: Alice; Age: 34; Sex: F}}''. This transformation allows us to treat structured data as natural language sentences, making it directly compatible with the documents and consumable by attention modules.

\stitle{2. Sentence Encoder:} We employ a pre-trained sentence encoder, $\xi(\cdot)$, which maps both the linearized row strings and the sentences from the document into embeddings:
\begin{equation*}
\resizebox{\linewidth}{!}{$
\mathbf{R} = \left[ \xi(\operatorname{linearize}(T)) \right]^{\top} \in \mathbb{R}^{n \times d}; \quad
\mathbf{S} = [\xi(s_1), \ldots, \xi(s_m)]^{\top} \in \mathbb{R}^{m \times d}
$}
\end{equation*}
This yields two matrices $\mathbf{R}$ and $\mathbf{S}$ of initial, \textit{non-contextualized} embeddings. Each row in $\mathbf{R}$ is a vector representing the semantic essence of a corresponding table row (e.g., the first row vector represents the record for \ex{\textit{Alice}}), and each row in $\mathbf{S}$ is a vector for a sentence in a document $D_i$. These initial vectors capture the general meaning of each item in isolation but lack any awareness of the specific context of the other modality. The weights of the base encoder $\xi$ are kept \textbf{frozen} to leverage its powerful, general-purpose linguistic knowledge.

\subsection{Stage 2: Bidirectional Contextualization}

The centerpiece of the LOKI pipeline is its hierarchical bidirectional cross-attention module. Unlike traditional unidirectional attention where context flows from a source to a target, our architecture is designed around the premise that meaningful alignment requires a symmetric exchange of information. A table row's meaning is grounded by the sentences that mention its entities, and a sentence's relevance is determined by the tabular data it references. This stage produces \textit{contextualized cross-modal representations}.

The module consists of two parallel cross-attention blocks, stabilized by a \textit{\textbf{gated attention mechanism}}~\cite{abs-2505-06708} that helps prevent attention collapse. We retain the Forward Attention Matrix $\mathbf{A}_f$ and Reverse Attention Matrix $\mathbf{A}_r$ as the internal attention distributions of these blocks. For a given set of queries ($\mathbf{Q}$), keys ($\mathbf{K}$), and values ($\mathbf{V}$), the attention matrix $\mathbf{A}$ and its output $\mathbf{H}$ are computed as:
\begin{gather*}
\mathbf{A}(\mathbf{Q},\mathbf{K})
=
\operatorname{softmax}\left(
\frac{
(\mathbf{Q}\mathbf{W}_Q)
(\mathbf{K}\mathbf{W}_K)^{\top}
}{
\sqrt{d_k}
}
\right);
\\
\mathbf{H}(\mathbf{Q},\mathbf{K},\mathbf{V})
=
\mathbf{A}(\mathbf{Q},\mathbf{K})
(\mathbf{V}\mathbf{W}_V)
\end{gather*}
where $\mathbf{W}_Q$, $\mathbf{W}_K$, and $\mathbf{W}_V$ are the query, key, and value projection matrices, respectively, and $d_k$ is the dimensionality of the projected keys. These projection matrices are shared between the forward and reverse cross-attention blocks, providing a common parameterization for both directions. To enable parameter-efficient task-specific adaptation, we apply Low-Rank Adaptation (LoRA) to the shared projection matrices while keeping the base encoder $\xi$ frozen. This allows the cross-attention module to learn task-specific interactions between rows and sentences without modifying the encoder's general-purpose semantic representations.

\stitle{1. Forward Attention (Rows $\rightarrow$ Sentences):} In the top block, table rows act as queries to seek information from the sentences, which serve as keys and values. This produces contextualized row representations $\widetilde{\mathbf{R}}$, enriched by the relevant sentence context:
\begin{equation*}
\mathbf{A}_f
=
\mathbf{A}(\mathbf{R},\mathbf{S});
\quad
\mathbf{H}_f
=
\mathbf{H}(\mathbf{R},\mathbf{S},\mathbf{S});
\quad
\widetilde{\mathbf{R}}
=
\mathbf{R}
+
\mathbf{H}_f
\odot
\sigma(\mathbf{R}\mathbf{W}_g^f)
\end{equation*}
This operation contextualizes each row using the sentences most relevant to it. In our running example, the \ex{\textit{Alice}} row attends most strongly to the sentence \ex{$s_1$} describing her \ex{\textit{Vancomycin}} prescription, producing a sentence-aware representation in $\widetilde{\mathbf{R}}$. The residual connection ($\mathbf{R}+$) preserves the row's original identity.

\stitle{2. Reverse Attention (Sentences $\rightarrow$ Rows):} Symmetrically, the bottom block uses sentences as queries to attend to the table rows. This process produces the contextualized sentence representations $\widetilde{\mathbf{S}}$, enriched by the relevant row context:
\begin{equation*}
\mathbf{A}_r
=
\mathbf{A}(\mathbf{S},\mathbf{R});
\quad
\mathbf{H}_r
=
\mathbf{H}(\mathbf{S},\mathbf{R},\mathbf{R});
\quad
\widetilde{\mathbf{S}}
=
\mathbf{S}
+
\mathbf{H}_r
\odot
\sigma(\mathbf{S}\mathbf{W}_g^r)
\end{equation*}
Here, $\mathbf{W}_g^f$ and $\mathbf{W}_g^r$ are separately learned gating parameters for the forward and reverse directions. This operation contextualizes each sentence with the rows it references. The sentence \ex{$s_1$} describing \ex{\textit{Alice}}'s \ex{\textit{Vancomycin}} prescription attends most strongly to the corresponding patient and medication rows, producing a row-aware representation in $\widetilde{\mathbf{S}}$. Together, the two directions resolve ambiguity by conditioning each modality on the other.

\subsection{Stage 3: Scoring and Aggregation}
\label{Stage-3}

With the bidirectionally contextualized representations, the pipeline computes its two primary outputs.

\stitle{Pair-Score Matrix:} The fine-grained semantic alignment between individual rows and sentences is captured in the pair-score matrix $\mathbf{P}\in\mathbb{R}^{n\times m}$, computed using cosine similarity between their contextualized representations. Here, $r\in\{1,\ldots,n\}$ indexes the table rows, corresponding to the rows of $\mathbf{P}$, while $s\in\{1,\ldots,m\}$ indexes the sentences, corresponding to its columns:
\begin{equation*}
P_{rs}
=
\frac{
\langle\widetilde{\mathbf{R}}_r,\widetilde{\mathbf{S}}_s\rangle
}{
\|\widetilde{\mathbf{R}}_r\|_2
\cdot
\|\widetilde{\mathbf{S}}_s\|_2
}
\end{equation*}
The pair-score matrix preserves the row-sentence granularity required for join-path extraction. In our running example, the \ex{\textit{Alice}} row receives a high score for sentence \ex{$s_1$} describing her prescription and lower scores with sentences concerning unrelated patients.

\stitle{Global Similarity Aggregation:} For the global retrieval task and loss calculation, $\mathbf{P}$ is aggregated into a scalar similarity score, $\operatorname{Sim}(T,D)$. Based on empirical validation, we adopt \textbf{Top-$K$ sum pooling} with $K=5$ by default:
\begin{equation*}
\operatorname{Sim}(T,D)
=
\sum_{(r,s)\in\operatorname{TopK}(\mathbf{P};K)}
P_{rs}
\end{equation*}
Here, $\operatorname{TopK}(\mathbf{P};K)$ denotes the index pairs $(r,s)$ corresponding to the $K$ largest entries of $\mathbf{P}$. By aggregating only the strongest row-sentence links, this strategy avoids relying on a single pair, as in max-pooling, while preventing informative signals from being diluted by mean-pooling. It also concentrates the global ranking gradient on the most relevant local interactions, directly coupling table-text retrieval with fine-grained row-sentence alignment.

\subsection{Stage 4: Self-Supervised Learning Objective}

LOKI's training (Fig.~\ref{fig:LOKI-Training-Pipeline}) utilizes a composite loss function defined over triplets of the form $(T, D^+, D^-)$, where $D^+$ denotes a semantically relevant document for table $T$ and $D^-$ denotes an unrelated or hard-negative document. The training objective jointly optimizes five complementary behaviors in the total loss:
\begin{equation*}
\begin{split}
\mathcal{L}_{\mathrm{total}} = 
& \bar{\lambda}_{\mathrm{rank}}\,\mathcal{L}_{\mathrm{rank}}
+ \bar{\lambda}_{\mathrm{distill}}\,\mathcal{L}_{\mathrm{distill}}
+ \bar{\lambda}_{\mathrm{pair}}\,\mathcal{L}_{\mathrm{pair}} \\
& + \underbrace{
\bar{\lambda}_{\mathrm{sig}}\,\mathcal{L}_{\mathrm{sig}}
+ \bar{\lambda}_{\mathrm{sink}}\,\mathcal{L}_{\mathrm{sink}}
}_{\text{Regularization Terms}}
\end{split}
\end{equation*}
Here, $\mathcal{L}_{\mathrm{rank}}$ drives coarse-grained table-document retrieval using the aggregated positive and negative pair scores, $\mathcal{L}_{\mathrm{distill}}$ aligns LOKI's pair-score distributions with the frozen-encoder's similarity distributions, and $\mathcal{L}_{\mathrm{pair}}$ sharpens fine-grained row-sentence separation within the pair score matrix. The final two components, $\mathcal{L}_{\mathrm{sig}}$ and $\mathcal{L}_{\mathrm{sink}}$, act as regularization losses over the contextualized representations and the bidirectional attention maps. The loss coefficients are normalized to sum to $1.0$ before aggregation.

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/LOKI-Training.pdf}
    \caption{LOKI Training: Coarse-to-Fine Grained Alignment.}
  \label{fig:LOKI-Training-Pipeline}
\end{figure}

\stitle{1. Global Ranking Loss ($\mathcal{L}_{\mathrm{rank}}$):} The global objective encourages the positive table-document pair to receive a higher aggregated similarity than the negative pair:
\begin{equation*}
\mathcal{L}_{\mathrm{rank}}
=
-\log
\frac{\exp(\operatorname{Sim}(T,D^+)/\tau)}
{\exp(\operatorname{Sim}(T,D^+)/\tau)+\exp(\operatorname{Sim}(T,D^-)/\tau)}
\end{equation*}
where $\tau$ is a temperature parameter that controls the sharpness of the contrastive comparison between positive and negative table-document pairs; we used $\tau=0.2$ by default. Since $\operatorname{Sim}(T,D)$ is aggregated from the pair-score matrix, this objective propagates table-text supervision to the strongest row-sentence interactions.

\stitle{2. Pair-Score Distillation Loss ($\mathcal{L}_{\mathrm{distill}}$):} Because the global ranking objective uses Top-$K$ aggregation, its supervision is concentrated on the strongest row-sentence pairs. We therefore distill the broader similarity structure of the frozen encoder into LOKI's pair-score matrix $\mathbf{P}$. This does not require a separate teacher model. The teacher scores are the cosine similarities between the original non-contextualized embeddings $\mathbf{R}$ and $\mathbf{S}$. To reduce the influence of generic sentences that are similar to many rows, we center each teacher score by the mean score received by its sentence:
\begin{equation*}
P^{\xi}_{rs}
=
\frac{\langle \mathbf{R}_r,\mathbf{S}_s\rangle}
{\|\mathbf{R}_r\|\cdot\|\mathbf{S}_s\|};
\qquad
\widehat{P}^{\xi}_{rs}
=
P^{\xi}_{rs}
-
\frac{1}{n}\sum_{r'=1}^{n}P^{\xi}_{r's}
\end{equation*}
We then construct two conditional distributions from the centered teacher scores and the contextualized student scores:
\begin{equation*}
\begin{aligned}
\mathbf{D}^{\xi}_{\mathbf{R}\rightarrow\mathbf{S}}
&=
\operatorname{softmax}_{s}\left(\frac{\widehat{\mathbf{P}}^{\xi}}{\tau_t}\right);
\quad
\mathbf{D}^{\mathrm{LOKI}}_{\mathbf{R}\rightarrow\mathbf{S}}
=
\operatorname{softmax}_{s}\left(\frac{\mathbf{P}}{\tau_s}\right);
\\
\mathbf{D}^{\xi}_{\mathbf{S}\rightarrow\mathbf{R}}
&=
\operatorname{softmax}_{r}\left(\frac{\widehat{\mathbf{P}}^{\xi}}{\tau_t}\right);
\quad
\mathbf{D}^{\mathrm{LOKI}}_{\mathbf{S}\rightarrow\mathbf{R}}
=
\operatorname{softmax}_{r}\left(\frac{\mathbf{P}}{\tau_s}\right)
\end{aligned}
\end{equation*}
Here, $\operatorname{softmax}_{s}$ normalizes over sentences for each row, whereas $\operatorname{softmax}_{r}$ normalizes over rows for each sentence. We use teacher and student temperatures $\tau_t=0.5$ and $\tau_s=0.1$, respectively. LOKI matches the teacher and student distributions in both normalization directions using Jensen-Shannon divergence:
\begin{equation*}
\mathcal{L}_{\mathrm{distill}}
=
\frac{1}{2}
\left[
\operatorname{JS}\!\left(
\mathbf{D}^{\xi}_{\mathbf{R}\rightarrow\mathbf{S}}
\,\|\, 
\mathbf{D}^{\mathrm{LOKI}}_{\mathbf{R}\rightarrow\mathbf{S}}
\right)
+
\operatorname{JS}\!\left(
\mathbf{D}^{\xi}_{\mathbf{S}\rightarrow\mathbf{R}}
\,\|\, 
\mathbf{D}^{\mathrm{LOKI}}_{\mathbf{S}\rightarrow\mathbf{R}}
\right)
\right]
\end{equation*}
The first term preserves each row's relative alignment across sentences, while the second preserves each sentence's relative alignment across rows. We compute this loss for both positive and negative table-document contexts and average the results. This preserves alignment structure beyond the strongest Top-$K$ pairs without directly supervising the internal attention matrices $\mathbf{A}_f$ and $\mathbf{A}_r$.
% \stitle{2. Attention Distillation Loss ($\mathcal{L}_{\mathrm{distill}}$):} The ranking objective may over-focus on a small number of salient pairs. We therefore use the frozen encoder as a teacher to preserve its broader alignment structure. Teacher scores are computed from the original embeddings, while student scores are obtained from $\mathbf{P}$:
% \begin{equation*}
% \begin{aligned}
% \mathbf{P}^{\xi}_{ij}
% &=
% \frac{\langle \mathbf{R}_i,\mathbf{S}_j\rangle}
% {\|\mathbf{R}_i\|\cdot\|\mathbf{S}_j\|}; \enspace
% \mathbf{D}^{\xi}
% =
% \operatorname{softmax}\left(\frac{\mathbf{P}^{\xi}}{\tau_t}\right); \enspace
% \mathbf{D}^{\mathrm{LOKI}}
% =
% \operatorname{softmax}\left(\frac{\mathbf{P}}{\tau_s}\right)
% \end{aligned}
% \end{equation*}
% Hub-centering is applied to the teacher scores before row-wise and column-wise normalization. LOKI then matches the teacher distributions in both directions using Jensen-Shannon divergence:
% \begin{equation*}
% \mathcal{L}_{\mathrm{distill}}
% =
% \frac{1}{2}
% \left[
% \operatorname{JS}\!\left(
% \mathbf{D}^{\xi}_{\mathbf{R}\rightarrow\mathbf{S}}
% \,\|\, 
% \mathbf{D}^{\mathrm{LOKI}}_{\mathbf{R}\rightarrow\mathbf{S}}
% \right)
% +
% \operatorname{JS}\!\left(
% \mathbf{D}^{\xi}_{\mathbf{S}\rightarrow\mathbf{R}}
% \,\|\, 
% \mathbf{D}^{\mathrm{LOKI}}_{\mathbf{S}\rightarrow\mathbf{R}}
% \right)
% \right]
% \end{equation*}
% This preserves broader cross-modal structure while reducing attention concentration on generic rows or sentences.

\stitle{3. Local Pairwise Loss ($\mathcal{L}_{\mathrm{pair}}$):} To sharpen fine-grained alignment, we contrast the positive and negative pair-score matrices for each training triplet:
\begin{equation*}
\mathcal{L}_{\mathrm{pair}}
=
\frac{1}{|\Omega|}
\sum_{(r,s)\in\Omega}
\max\Big\{
0,\,
m_{\mathrm{pair}}
-
\big(
P^+_{rs}
-
P^-_{rs}
\big)
\Big\}
\end{equation*}
where $r$ and $s$ index table rows and sentence positions, respectively, and $\Omega$ contains the valid row-sentence positions over which $\mathbf{P}^+$ and $\mathbf{P}^-$ are compared. We use a local margin of $m_{\mathrm{pair}}=0.3$ by default. The loss encourages row-sentence interactions in the positive context to score higher than those in the negative context by at least this margin. The resulting loss is averaged over the training triplets. This term sharpens the final pair-score matrix \textbf{\textit{without requiring any ground-truth row-sentence alignment labels}} and complements the global ranking loss by enforcing local discriminability between positive and negative contexts.

\stitle{4. Regularization Losses ($\mathcal{L}_{\mathrm{sig}}$, $\mathcal{L}_{\mathrm{sink}}$):} We use two complementary regularizers to prevent representation and attention collapse. First, SIGReg~\cite{SIGRegLeCun2025} encourages diversity and approximate isotropy in the contextualized embeddings by penalizing deviations of their random projections from a Gaussian distribution:
\begin{equation*}
\mathcal{L}_{\mathrm{sig}}
=
\frac{1}{4}
\Big[
\operatorname{SIGReg}(\widetilde{\mathbf{R}}^+)
+
\operatorname{SIGReg}(\widetilde{\mathbf{S}}^+)
+
\operatorname{SIGReg}(\widetilde{\mathbf{R}}^-)
+
\operatorname{SIGReg}(\widetilde{\mathbf{S}}^-)
\Big]
\end{equation*}
Second, a Sinkhorn-inspired marginal constraint~\cite{SinkhornAude2018} discourages hub-like attention, in which a small number of rows or sentences absorb most of the attention mass:
\begin{equation*}
\begin{aligned}
\operatorname{Sk}(\mathbf{A})
&=
\frac{1}{N_k}
\left\|
\operatorname{col\_sum}(\mathbf{A})
-
\frac{N_q}{N_k}\mathbf{1}
\right\|_2^2
+
\operatorname{Var}\!\left(
\operatorname{col\_sum}(\mathbf{A})
\right);
\\
\mathcal{L}_{\mathrm{sink}}
&=
\frac{1}{4}
\Big[
\operatorname{Sk}(\mathbf{A}^+_f)
+
\operatorname{Sk}(\mathbf{A}^+_r)
+
\operatorname{Sk}(\mathbf{A}^-_f)
+
\operatorname{Sk}(\mathbf{A}^-_r)
\Big]
\end{aligned}
\end{equation*}
Here, $\operatorname{col\_sum}(\mathbf{A})$ denotes the column sums of the row-normalized attention matrix, while $N_q$ and $N_k$ denote the numbers of valid queries and keys, respectively. The target column sum $N_q/N_k$ corresponds to distributing the attention mass uniformly across the keys. Together, these regularizers maintain diverse contextualized representations and balanced bidirectional attention distributions.


\subsection{Stage 5: Join Path Extraction}

The subsequent stage of the LOKI pipeline shifts from training to inference-time join-path extraction. We denote the resulting trained model by $\operatorname{LOKI}_{\theta}$, where $\theta$ represents its learned parameters while the encoder $\xi$ remains frozen. The trained model uses the global similarity score defined in Section~\ref{Stage-3} to retrieve candidate table-document pairs from an unseen data lake. For any document $D$, two schematically disjoint tables $T_A$ and $T_B$ form a candidate combination when both are independently retrieved as relevant to $D$. Stage 5 therefore operates on combinations discovered by $\operatorname{LOKI}_{\theta}$. For each resulting candidate combination $(T_A,D,T_B)$, $\operatorname{LOKI}_{\theta}$ jointly contextualizes the rows from both tables with the sentences in $D$ while preserving their table of origin. Rather than processing each table independently, we linearize their rows and concatenate the resulting sequences in a fixed order:
\begin{equation*}
\mathbf{R}_0 = \xi\big(\operatorname{linearize}(T_A) \oplus \operatorname{linearize}(T_B)\big);
\quad
\mathbf{S}_0 = \xi\big(\operatorname{sentences}(D)\big)
\end{equation*}
where $\oplus$ denotes ordered concatenation, such that the first $n_A$ rows originate from $T_A$ and the following $n_B$ rows from $T_B$. A single forward pass then produces the contextualized representations and pair-score matrix:
\begin{equation*}
(\widetilde{\mathbf{R}},\widetilde{\mathbf{S}},\mathbf{P})
=
\operatorname{LOKI}_{\theta}(\mathbf{R}_0,\mathbf{S}_0)
\end{equation*}
These outputs provide a shared row-sentence context from which sparse, evidence-backed join paths can be extracted. Algorithm~\ref{algo:inference-loki} summarizes this join path extraction process.

\stitle{1. Atomic Link Identification:}
The pair-score matrix $\mathbf{P}$ is dense because every row in the ordered sequence $\mathbf{R}_0$ receives an affinity score against every sentence in $D$. Since only a small subset provides useful evidence for text-mediated join paths, $\operatorname{LOKI}_{\theta}$ converts $\mathbf{P}$ into a sparse set of high-confidence atomic links. For each candidate combination $(T_A,D,T_B)$, we compute an adaptive threshold $\gamma$ rather than using a globally fixed cutoff. For each row $r$, let $q_r=\max_s(P_{rs})$ denote its highest score across all sentences, and let $P_{75}$ denote the 75th percentile of $\{q_r\}_{r=1}^{n_A+n_B}$. Furthermore, $\mu_{\mathbf{P}}$ and $\sigma_{\mathbf{P}}$ denote the mean and standard deviation of all entries in $\mathbf{P}$. The adaptive threshold is given by:
\begin{equation*}
\gamma
=
\max\!\left(
\min\!\left(
P_{75},
\mu_{\mathbf{P}}+2\sigma_{\mathbf{P}}
\right),
\gamma_{\min}
\right)
\end{equation*}
where $\gamma_{\min}=0.15$ is the default minimum score threshold. This makes the extraction stricter when the example contains clear row-sentence alignments, while still preventing the threshold from collapsing on noisier examples. We then apply mutual Top-$k$ filtering. For each row $r_i$, the filter retains the indices of its $k_r$ highest-scoring sentences, whereas for each sentence $s_t$, it retains the indices of its $k_s$ highest-scoring rows:
\begin{equation*}
\mathcal{N}^{\mathrm{row}}_{k_r}(i)
=
\operatorname{Top}_{k_r}(P_{i,:});
\quad
\mathcal{N}^{\mathrm{sent}}_{k_s}(t)
=
\operatorname{Top}_{k_s}(P_{:,t})
\end{equation*}
where $\operatorname{Top}_k(\cdot)$ returns the indices of the $k$ largest entries. The sentence-side operation is applied independently to the row partitions of $T_A$ and $T_B$. We use $k_r=32$ and $k_s=10$ by default. The row-side filter prevents a row from attaching to too many vague sentences, while the sentence-side filter suppresses hub sentences that align weakly with many rows but do not provide discriminative evidence for a specific join path. The resulting atomic-link set is:
\begin{equation*}
\mathcal{J}
=
\left\{
(i,t)
\;\middle|\;
P_{it}\geq\gamma
\;\land\;
t\in\mathcal{N}^{\mathrm{row}}_{k_r}(i)
\;\land\;
i\in\mathcal{N}^{\mathrm{sent}}_{k_s}(t)
\right\}
\end{equation*}
Since Stage 5 must ultimately connect rows across two schematically disjoint tables, we partition these links by table origin:
\begin{equation*}
    \begin{aligned}
    \mathcal{J}_A &= \{(i,t)\in\mathcal{J}:1\le i\le n_A\} \\
    \mathcal{J}_B &= \{(j,t):(n_A+j,t)\in\mathcal{J},\;1\le j\le n_B\}
\end{aligned}
\end{equation*}
Here, $\mathcal{J}_A$ and $\mathcal{J}_B$ preserve table origin while retaining the sentence supporting each atomic link. These table-specific links provide the evidence anchors for constructing cross-table semantic join paths.
% Thus, $\mathcal{J}_A$ contains row-sentence links from $T_A$, while $\mathcal{J}_B$ contains row-sentence links from $T_B$. Each surviving atomic link remains directly interpretable because it retains the original evidence sentence. In the running example, the sentence ``\ex{\textit{Alice Johnson was prescribed Lisinopril to manage her hypertension.}}'' should survive as an atomic link to the \ex{\textit{Alice Johnson}} row in the \ex{\textit{Patients}} table and also as an atomic link to the \ex{\textit{Lisinopril}} row in the \ex{\textit{Medications}} table. These two table-specific atomic links become the evidence anchors used by the next step to construct a cross-table semantic join path.

\begin{algorithm}[]
\SetAlgoLined
\KwIn{Retrieved candidate $(T_A,D,T_B)$, frozen encoder $\xi$, trained model $\operatorname{LOKI}_{\theta}$, threshold floor $\gamma_{\min}$, and Top-$k$ parameter $k$}
\KwOut{Atomic links $\mathcal{J}_A,\mathcal{J}_B$ and candidate join paths $\mathcal{P}_{\mathrm{cand}}$}
\BlankLine

\tcp{\textbf{Step 1: Joint row-sentence encoding}}
$\mathbf{R}_0 \leftarrow \xi\!\left(\operatorname{linearize}(T_A)\oplus\operatorname{linearize}(T_B) \right)$ \;
$\mathbf{S}_0 \leftarrow \xi(\operatorname{sentences}(D))$ \;
$(\tilde{\mathbf{R}},\tilde{\mathbf{S}},\mathbf{P}) \leftarrow \operatorname{LOKI}_{\theta}(\mathbf{R}_0,\mathbf{S}_0)$ \;

\tcp{\textbf{Step 2: Compute adaptive score floor}}
$\gamma \leftarrow
\max\!\left(
\min\!\left(P_{75},\mu_{\mathbf{P}}+2\sigma_{\mathbf{P}}\right),
\gamma_{\min}
\right)$ \;

\tcp{\textbf{Step 3: Extract table-specific atomic links}}
$\mathcal{N}^{\mathrm{row}}_{k_r}(i)\leftarrow \operatorname{Top}_{k_r}(P_{i,:}), \quad
\mathcal{N}^{\mathrm{sent}}_{k_s}(t)\leftarrow \operatorname{Top}_{k_s}(P_{:,t})$ \;

$\mathcal{J}\leftarrow
\{(i,t)\mid
P_{it}\ge\gamma
\land t\in\mathcal{N}^{\mathrm{row}}_{k_r}(i)
\land i\in\mathcal{N}^{\mathrm{sent}}_{k_s}(t)$ \;

$\mathcal{J}_A\leftarrow\{(i,t)\in\mathcal{J}:1\le i\le n_A\}$ \;
$\mathcal{J}_B\leftarrow\{(j,t):(n_A+j,t)\in\mathcal{J},\;1\le j\le n_B\}$ \;

\tcp{\textbf{Step 4: Construct shared-sentence join paths}}
$\mathcal{P}_{\mathrm{cand}}\leftarrow
\left\{
(r_i^A,s_t,r_j^B)
\;\middle|\;
(i,t)\in\mathcal{J}_A
\land
(j,t)\in\mathcal{J}_B
\right\}$ \;

Rank paths $\mathcal{P}_{\mathrm{cand}}$ by bridge score and keep strongest candidates \;
\Return{$\mathcal{J}_A,\mathcal{J}_B,\mathcal{P}_{\mathrm{cand}}$}
\caption{LOKI's inference-time join path extraction}
\label{algo:inference-loki}
\end{algorithm}

\begin{figure*}[]
  \centering
  \includegraphics[width=\linewidth]{figures/Example_Integration.pdf}
    \caption{LOKI inference pipeline for join-path extraction and semantic materialization. (a) Given a retrieved candidate combination $(T_A,D,T_B)$, a single joint forward pass through the trained model $\operatorname{LOKI}_{\theta}$ produces the pair-score matrix $\mathbf{P}$. High-confidence atomic links from $\mathbf{P}$ are composed into candidate join paths, (b) whose contextual representations are clustered into the illustrative groups $\{C_1,C_3\}$. (c) The Generalization Function $G$ assigns the descriptive relationship labels $\{R_1,R_3\}$, (d) and the labeled clusters are materialized as relation-specific integrated tables with supporting evidence.}
  \label{fig:example_integration}
\end{figure*}

\stitle{2. Transitive Join-Path Construction:}
Because $T_A$ and $T_B$ are schematically disjoint, LOKI does not assume that a row from one table can be joined directly with a row from the other table. Instead, the connection must be mediated by text. After atomic-link identification, a row $r_i^A\in T_A$ and a row $r_j^B\in T_B$ become join candidates only when they share at least one mediating sentence $s_t$. For each shared sentence, LOKI constructs a text-mediated join path and assigns it a bridge weight:
\begin{equation*}
p_{ijt} = (r_i^A,s_t,r_j^B), \quad w_{ijt} = \frac{ P_{it}+P_{n_A+j,t} }{2}
\end{equation*}
Here, $p_{ijt}$ is a single-evidence instance of the general semantic join path $p=(r_i^A,S_p,r_j^B)$, with $S_{p_{ijt}}=\{s_t\}$. Paths connecting the same row pair and relationship type are consolidated by collecting their mediating sentences into $S_p$ during semantic materialization. For simplicity, each path in our running example contains a single sentence. Because a candidate path is formed only when $s_t$ has retained atomic links to both rows, $w_{ijt}$ summarizes their joint compatibility and serves as the bridge confidence used to rank candidate paths and weight the contextualized sentence representation during semantic materialization. The candidate path set is then:
\begin{equation*}
\mathcal{P}_{\mathrm{cand}} = \left\{ p_{ijt} = (r_i^A,s_t,r_j^B) \;\middle|\; (i,t)\in\mathcal{J}_A \wedge (j,t)\in\mathcal{J}_B\right\}
\end{equation*}
To avoid over-representing repeated or generic evidence, LOKI retains only the strongest paths per sentence and per row pair. The resulting $\mathcal{P}_{\mathrm{cand}}$ is therefore a compact set of explicit, evidence-backed bridges. In the running example, the sentences \ex{$\{s_1,\ldots,s_5\}$} produce the following paths: \ex{\textit{$p_1=(I_1,\{s_1\in D_1\},M_1)$}}, \ex{\textit{$p_2=(I_1,\{s_2\in D_1\},M_1)$}}, \ex{\textit{$p_3=(I_1,\{s_3\in D_1\},M_1)$}}, \ex{\textit{$p_4=(I_1,\{s_4\in D_1\},M_2)$}}, and \ex{\textit{$p_5=(I_1,\{s_5\in D_1\},M_3)$}}, respectively.
% Each element of $\mathcal{P}_{\mathrm{cand}}$ is therefore an explicit semantic bridge between the two tables, supported by a concrete sentence from $D$. To avoid over-representing broad sentences or repeated evidence, LOKI ranks paths by their bridge score and retains only a bounded number of strongest row pairs per sentence and strongest evidence sentences per row pair. The output of Stage 5 is consequently a compact set of evidence-backed path triples, rather than a direct joined table. In the running example, the sentence ``\ex{\textit{Alice Johnson was prescribed Lisinopril to manage her hypertension.}}'' becomes a transitive bridge because it links to both the \ex{\textit{Alice Johnson}} row in $T_A$ and the \ex{\textit{Lisinopril}} row in $T_B$, therefore producing the semantic join path \ex{\textit{$p_1=(I_1,\{s_1\in D_1\},M_1)$}}, which is then passed to Stage 6 for relationship labeling and materialization.

\subsection{Stage 6: Semantic Materialization}
\label{sec:materialization}

The discovery-driven integration problem in Section~\ref{sec:problem_statement} requires mapping candidate join paths to latent relationship types $\mathcal{R}$, and materializing them as typed integrated tables $\mathcal{T}$. Each candidate path $p_{ijt}=(r_i^A,s_t,r_j^B)\in\mathcal{P}_{\mathrm{cand}}$ is treated as a distinct evidence unit, allowing different sentences connecting the same row pair to express different relationships. In the running example, \ex{$p_1=(I_1,\{s_1\in D_1\},M_1)$} and \ex{$p_2=(I_1,\{s_2\in D_1\},M_1)$} share the same row pair but express \ex{\textit{Prescribed\_For}} and \ex{\textit{Adverse\_Effect}}, respectively.

\stitle{1. Path Representation and Clustering:}
To group candidate paths by the relationship expressed in their mediating evidence, LOKI constructs a path-specific representation that combines the contextualized sentence with the strength of its attachment to both table rows. For a candidate path $p_{ijt}=(r_i^A,s_t,r_j^B)$, let
\begin{equation*}
    \alpha_{it}=P_{it},
    \quad
    \beta_{jt}=P_{n_A+j,t},
    \quad
    w_{ijt}=\frac{\alpha_{it}+\beta_{jt}}{2}
\end{equation*}
Here, $\alpha_{it}$ measures how strongly sentence $s_t$ supports row $r_i^A$, $\beta_{jt}$ measures how strongly it supports row $r_j^B$, and $w_{ijt}$ is the average of these scores, representing the confidence of the complete bridge. Before applying these weights, we $L_2$-normalize the contextualized embeddings so that the three components begin on the same scale. Any subsequent difference in their contributions is therefore introduced by the alignment scores rather than by differences in the original embedding norms. An unweighted concatenation would treat the two rows and the sentence as equally important, even when one of the underlying links is considerably weaker. We instead use the alignment scores as multiplicative gates:
\begin{equation*}
\boldsymbol{\phi}^{\mathrm{ctx}}(p_{ijt})
=
\left[
\alpha_{it}\widetilde{\mathbf{r}}_i^A
\;\Vert\;
w_{ijt}\widetilde{\mathbf{s}}_t
\;\Vert\;
\beta_{jt}\widetilde{\mathbf{r}}_j^B
\right]
\in\mathbb{R}^{3d}
\end{equation*}
The ordered concatenation preserves the distinct roles of the two table rows and the mediating sentence. Meanwhile, the weights increase or reduce the contribution of each component according to the strength of its supporting evidence. In particular, $\alpha_{it}$ and $\beta_{jt}$ preserve potentially asymmetric attachment strengths, while $w_{ijt}$ controls the contribution of the sentence according to the confidence of the overall bridge. The weighting does not create a new embedding space; it changes the position of each path within the concatenated space according to its evidence. Thus, paths involving the same sentence remain distinguishable when they connect different row pairs or exhibit different attachment strengths. Finally, the complete path vector is $L_2$-normalized before clustering, preserving these relative contributions while preventing its overall magnitude from dominating the clustering distance:
\begin{equation*}
    \mathcal{C}
    =
    \{C_1,\ldots,C_K\}
    =
    \operatorname{HDBSCAN}
    \left(
    \left\{
    \boldsymbol{\phi}^{\mathrm{ctx}}(p)
    \mid
    p\in\mathcal{P}_{\mathrm{cand}}
    \right\}
    \right)
\end{equation*}
Each cluster $C_k$ therefore groups text-mediated join paths whose row-conditioned evidence expresses similar relational semantics. In the running example, the paths \ex{$p_1$},  and \ex{$p_4$} are expected to be grouped together because they represent a \ex{\textit{Prescribed\_For}} relationship, while \ex{$p_3$} and \ex{$p_5$} form another group because they represent a \ex{\textit{Discontinued}} relationship.

\stitle{2. Relationship Materialization:}
After clustering, each cluster $C_k$ contains text-mediated join path paths whose row-conditioned evidence expresses a coherent but unnamed relationship. To make this relationship interpretable, we use a \textit{Generalization Function} $G$ that employs an LLM to summarize the shared evidence within the cluster and assign a descriptive relationship label $R_k$:
\begin{equation*}
    G:C_k\xrightarrow{\mathrm{LLM}}R_k
\end{equation*}
Each labeled cluster is then materialized as a relation-specific integrated table:
\begin{equation*}
    T_{\mathrm{integrated}}^{(R_k)}
    =
    \left\{
    (r_i^A,r_j^B,s_t)
    \;\middle|\;
    p_{ijt}=(r_i^A,s_t,r_j^B)\in C_k
    \right\}
\end{equation*}
Repeating this process for each labeled cluster produces the final set of relation-specific integrated tables. Accordingly, each integrated table is a relation-specific collection of evidence-backed links between $T_A$ and $T_B$, where every entry combines one record from $T_A$ with one record from $T_B$ and preserves the supporting evidence for the relationship $R_k$.
% The complete materialized output is the set of all such labeled cluster tables:
% \begin{equation*}
%     \mathcal{I}
%     =
%     \left\{
%     T_{\mathrm{integrated}}^{(R_k)}
%     \;\middle|\;
%     C_k\in\mathcal{C}
%     \right\}
%     =
%     T_A \mathrel{{\overset{\mathcal{P}}{\leadsto}}_{\mathcal{R}}} T_B
% \end{equation*}

The materialization process for a subset of the paths in our running example is illustrated in Fig.~\ref{fig:example_integration}. The illustrated candidate paths are first represented in the latent space and clustered into relation-consistent groups. The paths \ex{\textit{$p_1$}} and \ex{\textit{$p_3$}} remain close because they share the same row pair \ex{\textit{$(M_1,I_1)$}}, but they are assigned to different clusters because they represent different relationships. The Generalization Function then labels $C_1$ as \ex{\textit{$R_1:\text{Prescribed\_For}$}} and $C_2$ as \ex{\textit{$R_3:\text{Discontinued}$}}. Finally, each labeled cluster is materialized as a separate integrated table with sentence-level provenance.

% Algorithm~\ref{algo:semantic-materialization} summarizes this semantic materialization procedure.
% \begin{algorithm}[]
% \SetAlgoLined
% \KwIn{Candidate paths $\mathcal{P}_{\mathrm{cand}}$, contextualized rows $\tilde{\mathbf{R}}$, contextualized sentences $\tilde{\mathbf{S}}$, pair-score matrix $\mathbf{P}$, ontology $\mathcal{O}_{\mathcal{R}}$, Generalization Function $G$}
% \KwOut{Discovered relationship types $\mathcal{R}$ and typed integrated tables $\mathcal{T}$}
% \BlankLine

% \tcp{\textbf{Step 1: Cluster candidate paths}}
% $\Phi \leftarrow
% \left\{
% \boldsymbol{\phi}^{\mathrm{ctx}}(p)
% \mid
% p\in\mathcal{P}_{\mathrm{cand}}
% \right\}$ \;

% $\mathcal{C}\leftarrow
% \operatorname{HDBSCAN}(\Phi)$ \;

% \tcp{\textbf{Step 2: Label clusters and materialize tables}}
% $\mathcal{R}\leftarrow\emptyset,\quad \mathcal{T}\leftarrow\emptyset$ \;

% \ForEach{$C_k\in\mathcal{C}$}{
%     $R_k\leftarrow G(C_k,\mathcal{O}_{\mathcal{R}})$ \;

%     $T_{\mathrm{integrated}}^{(R_k)}
%     \leftarrow
%     \left\{
%     (r_i^A,r_j^B,s_t)
%     \;\middle|\;
%     p_{ijt}=(r_i^A,s_t,r_j^B)\in C_k
%     \right\}$ \;

%     $\mathcal{R}\leftarrow\mathcal{R}\cup\{R_k\}$ \;
%     $\mathcal{T}\leftarrow\mathcal{T}\cup\{T_{\mathrm{integrated}}^{(R_k)}\}$ \;
% }

% \Return{$\mathcal{R},\mathcal{T}$}
% \caption{LOKI's semantic materialization}
% \label{algo:semantic-materialization}
% \end{algorithm}

\stitle{\ex{Summary:}} LOKI's methodology follows a discovery-driven integration approach by turning text evidence into provenance-preserving integrated relations. Rather than forcing a direct schema-level join or returning black-box row-association scores, LOKI reconstructs a latent relational structure over disjoint tables. Each integrated table corresponds to a discovered relationship type in $\mathcal{R}$, and each entry remains traceable to the textual evidence that supports the cross-table relationship. The result is a queryable relational output whose semantics were not encoded in either input table, but recovered from the text that connects them.



==> old_introduction.tex <==
\section{Introduction}


Dimitris: I'll heavily revise the introduction.



\noindent\rule{\columnwidth}{1pt}

\stitle{The Missing Link}
Data lakes serve as centralized repositories for consolidating large volumes of heterogeneous data. These repositories often contain thousands of datasets, including structured tables and large collections of unstructured text that remain underutilized. Joining tables in this setting is difficult because datasets collected from disparate sources often lack compatible schemas, shared keys, or sufficient value overlap for relational joins \cite{GuoMHCG25,00020F25}. Two tables may contain related entities while sharing no overlapping columns. This prevents conventional joins and limits table-only join discovery methods \cite{Dong0NEO23,Koutras2025,GuoMHCG25}. In such cases, the missing relationships may instead be expressed in text \cite{AtaurRahman2026}. For example, a clinical note may reveal which drug treated a diagnosis, caused a complication, or was discontinued, although none of these relationships appears in the source tables. In a raw data lake, the relevant table pair, supporting documents, table-document associations, and relationship schema are not provided by default. This creates an \textbf{\textit{integration cold start}} in which neither the participating sources nor the missing relations are known in advance. Both must be discovered before the data can be joined, queried, and integrated.

\begin{tcolorbox}[boxrule=0.2pt, boxsep=0pt, colback=Snow1]
\stitle{Motivating Example:}
Consider the hospital data lake in Fig.~\ref{fig:motivating_example_loki}. It contains a collection of tables $\mathcal{T}$, that includes a \textit{Patients} table \ex{$T_1$}, a \textit{Medications} table \ex{$T_2$}, and a corpus $\mathcal{D}$ of \textit{Discharge Summaries}. The tables share no joinable attribute, and the lake provides neither table-document links nor a relationship schema. In \ex{$D_1$}, \ex{$s_1$} states that Alice Johnson (\ex{$I_1$}) received Vancomycin 1000 mg IV (\ex{$M_1$}), \ex{$s_2$} associates \ex{$M_1$} with nephrotoxicity, and \ex{$s_3$} records its discontinuation. Sentence \ex{$s_4$} records a separate prescription of Vancomycin 125 mg oral (\ex{$M_2$}) for a \textit{C.~difficile} infection, while \ex{$s_5$} states that Lisinopril (\ex{$M_3$}) was withheld because of acute kidney injury. Thus, \ex{$M_1$} and \ex{$M_2$} share a drug name but represent different medication usage patterns, while the same row pair \ex{$(M_1,I_1)$} expresses several relationships through different sentences. Discovery must determine the relevance of \ex{$D_1$} from these fine-grained row-sentence associations. Integration must then distinguish their semantics and materialize \ex{\textit{Prescribed\_For}}, \ex{\textit{Adverse\_Effect}}, and \ex{\textit{Discontinued}} relations without their types or a target schema being supplied in advance.
\end{tcolorbox}

\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{figures/Loki_Main_Example.pdf}
\caption{Discovery-driven integration within a data lake across multi-modal sources. Given disjoint \textit{Patients} and \textit{Medications} tables and \textit{Discharge Summaries}, coarse-grained approaches retrieve column-document pairs, whereas LOKI derives document relevance from fine-grained row-sentence associations. Existing integration systems require supplied entity-document links and predefined attributes or predicates. LOKI uses its discovered row-sentence associations to disambiguate and materialize evidence-backed cross-table relations without a predefined relationship type or target schema.}
\label{fig:motivating_example_loki}
\end{figure*}

% \stitle{The Problem}
% Existing data discovery approaches may retrieve related tables and documents, but they do not resolve which rows are related, which sentences support these row-level relationships, or which relationships they express. Schema and query-driven approaches can extract this information only after receiving inputs such as the relevant table-document pair, tuple-text keys, a latent relationship schema, or query predicates. In particular, the \textit{Patient-Diagnosis} table required for the next integration step does not yet exist and therefore cannot be supplied as an input. The lake must first be searched to retrieve the relevant tables and documents, align their rows and sentences, and materialize the discovered relationships as a \textit{Patient-Diagnosis} table. This newly materialized table can then expose further missing relationships with the \textit{Medication} table through sentence-level evidence. These relationships must be distinguished and materialized separately before the data can support a downstream analytical query, as shown in Fig.~\ref{fig:motivating_example_loki} (D).

\stitle{The Problem}
Existing multi-modal data \textbf{\textit{discovery}} approaches retrieve related tables and documents at a coarse-grained level, but they do not resolve which rows are related, which sentences support these row-level relationships, or what relationships they express. For instance, in Fig.~\ref{fig:motivating_example_loki}, CMDL~\cite{EltabakhKEA23} associates the \ex{$T_1.\textit{Name}$} and \ex{$T_2.\textit{Drug}$} columns with every relevant document in \ex{$\mathcal{D}$}. Existing schema and query-driven \textbf{\textit{integration}} approaches address a different problem in which inputs such as the relevant table-document pair, tuple-text keys, relationship schema, or query predicate are supplied in advance. THOR~\cite{RahmanN0S24} and ELEET~\cite{UrbanB24} populate the predefined \ex{\textit{Disease}} attribute for supplied patient-document links under the known relationship \ex{\textit{has\_disease}}, whereas ThalamusDB~\cite{JoT24} evaluates a supplied boolean predicate such as \ex{\textit{is\_diabetic}}.

In contrast, integrating disjoint tables from a raw multi-modal data lake is fundamentally more complex because their missing relational structure must first be discovered. Document relevance must be grounded in fine-grained row-sentence associations, which provide evidence for cross-table row-to-row connections. The resulting row-sentence-row paths must then be disambiguated before their relationship types can be inferred. In Fig.~\ref{fig:motivating_example_loki}, this requires distinguishing \ex{$M_1$} and \ex{$M_2$} despite their shared drug name, while materializing \ex{$(M_1, I_1)$} separately in the \ex{\textit{Prescribed\_For}}, \ex{\textit{Adverse\_Effect}}, and \ex{\textit{Discontinued}} relations using different evidence sentences.

% \stitle{Column-Valued Outputs Are Insufficient}
% Given \ex{$D_1$}, CMDL may retrieve the relevant diagnosis or medication column, whereas ELEET may populate such a column for a linked tuple. Neither output represents the distinct relational roles connecting the participating rows. For \ex{\textit{Vancomycin}}, such an output may return \ex{\textit{MRSA bacteremia}} and \ex{\textit{Acute Kidney Injury}}, but cannot express that Vancomycin \emph{Treats} the former, has an \emph{Adverse Effect}, and is \emph{Discontinued} because of the latter. Preserving these semantics would require predefined relationship-specific columns, thereby supplying the structure that must instead be discovered. Once collapsed into a shared column, these roles cannot be materialized separately or composed in later integration steps because their supporting context is lost. The required output is therefore a set of typed, sentence-grounded cross-table relations that remain explicit, queryable, and reusable.


\stitle{Challenges}
Realizing this task raises three challenges. \textbf{(C1) Lake-wide discovery}: must identify relevant table-document combinations from a large candidate space without a supplied target pair, table-document link, relation schema, or query. \textbf{(C2) Fine-grained disambiguation}: must recover row-sentence associations and distinguish among relationships involving the same tuple or row pair. Row-sentence links do not exist in data lakes and are prohibitively expensive to annotate. General-purpose encoders are not designed for row-sentence alignment. They often weaken the association between an attribute name and its value, limiting their ability to determine which row attributes a sentence refers to \cite{narayan2022can}. \textbf{(C3) Semantic materialization}: must compose local links into row-to-row paths, group them by the relationship expressed in their evidence, and materialize typed relational outputs with provenance.

\stitle{Proposed Solution}
We propose \textsf{\textbf{LOKI}} (Latent-space Optimization for Knowledge Integration), a hierarchical bidirectional cross-attention architecture based on \textbf{\textit{Discovery-Driven Integration}} paradigm. It discovers participating sources and reconstructs their missing relational structure before an analytical query can be formulated. \textbf{(C1)} LOKI derives global table-text similarity from fine-grained row-sentence evidence for lake-wide discovery. \textbf{(C2)} Its joint representation contextualizes rows and sentences together, learning these associations without row-sentence annotations and retaining the evidence needed to distinguish multiple relationships over the same row pair. \textbf{(C3)} During inference, it composes this evidence into sentence-grounded row-to-row paths and groups them by latent relationship semantics for typed, provenance-preserving materialization. LOKI therefore unifies source discovery, relationship disambiguation, and semantic materialization, transforming retrieved sources into reusable and queryable integrated tables.


% \stitle{Proposed Solution}
% We propose \textbf{LOKI} (Latent-space Optimization for Knowledge Integration), a hierarchical bidirectional cross-attention architecture for discovery-driven integration. \textbf{(C1)} LOKI learns global table-text similarity while preserving the row-sentence evidence underlying each score, enabling lake-wide source discovery. \textbf{(C2)} Its joint representation contextualizes rows and sentences with respect to one another, allowing fine-grained associations to emerge without row-sentence annotations and preserving the evidence needed to distinguish multiple relationships over the same row pairs. \textbf{(C3)} During inference, evidence from two discovered tables is composed into sentence-grounded row-to-row paths, grouped by their latent relationship semantics, and materialized as separate relations with provenance. LOKI therefore unifies source discovery, relationship disambiguation, and semantic materialization using the same learned representation, transforming retrieved sources into queryable integrated tables rather than treating retrieval as an isolated pre-processing step.

\medskip
\stitle{Contributions} This work makes the following primary contributions to the fields of multi-modal data discovery, integration, and representation learning:
\begin{itemize}[leftmargin=6mm]
\setlength\itemsep{1mm}

    \item \textbf{Discovery-Driven Integration.} We formulate a new data-management problem that starts from a raw multi-modal data lake without a target table pair, table-document links, a direct join key, a predefined relationship schema, or an analytical query. We formalize \textit{Semantic Join Path Discovery} as the discovery, disambiguation, and materialization of sentence-mediated row-to-row relations between schematically disjoint tables.

    \item \textbf{New Architecture for Joint Representation Learning.} We propose LOKI, a hierarchical bidirectional cross-attention architecture that learns contextualized row-sentence representations from coarse table-text supervision alone, enabling fine-grained alignments to emerge without explicit supervision.

    \item \textbf{State-of-the-Art Discovery and End-to-End Integration.} We evaluate LOKI progressively from implicit row-sentence alignment, to bidirectional table-text discovery, and finally to semantic integration. Across real-world benchmarks, LOKI significantly outperforms existing cross-modal discovery and representation-learning methods at data-lake scale, while its discovered paths form relation-consistent groups that can be materialized as typed, provenance-preserving tables.

\end{itemize}



==> old_problem.tex <==
\section{Preliminaries}

\subsection{Notations}

Let a raw multi-modal data lake be represented as $\mathcal{L}=(\mathcal{T},\mathcal{D})$, where $\mathcal{T}=\{T_k\}_{k=1}^{N}$ is a collection of tables and $\mathcal{D}=\{D_\ell\}_{\ell=1}^{M}$ is a collection of documents. Let a table be represented as a multiset of $n$ rows, \raisebox{0.3ex}{$T=\{r_i\}_{i=1}^{n}$}, conforming to a schema $\mathcal{S}=(c_1,\ldots,c_{|\mathcal{S}|})$, where $c_k$ is the $k^{\mathrm{th}}$ column. Similarly, let a document be represented as a multiset of $m$ sentences, \raisebox{0.3ex}{$D=\{s_j\}_{j=1}^{m}$}. We denote vectors in bold lowercase, $\mathbf{v}\in\mathbb{R}^d$ with dimension $d$, and matrices in bold uppercase, $\mathbf{M}$. The dot product is denoted by $\langle\cdot,\cdot\rangle$, element-wise multiplication by $\odot$, and the sigmoid function by $\sigma$.

\subsection{Task Formalization}

Our primary objective is to learn a function that, for each candidate table-document pair $(T,D)\in\mathcal{T}\times\mathcal{D}$, produces three key \textbf{outputs}:

\begin{enumerate}[leftmargin=6mm]
\setlength\itemsep{1mm}

    \item A \textbf{pair-score matrix}, $\mathbf{P} \in \mathbb{R}^{n \times m}$, where each entry $P_{ij}$ represents the fine-grained semantic relatedness between row $r_i$ and sentence $s_j$. This matrix is the substrate from which we extract text-mediated join paths and global similarity score.
   
    \item A \textbf{global similarity score}, $\operatorname{Sim}(T,D) \in \mathbb{R}$, derived from the pair-score matrix $\mathbf{P}$, which quantifies the overall semantic relevance between the table and the document. This score is used to compute the loss and to retrieve relevant table-document pairs from the data lake.

    \item A \textbf{set of atomic links}, $\mathcal{J} = \{(r_i, s_j) \mid P_{ij} \ge \gamma \}$, representing the sparse, high-precision connections between specific rows and sentences $(r_i \leftrightarrow s_j)$. These links are the fundamental building blocks used to materialize the semantic join paths.
\end{enumerate}

\noindent We formalize \textit{Text-Mediated Join Path}, the foundational task for our multi-modal discovery-driven integration as follows:

\begin{tcolorbox}[
    boxrule=1pt, 
    boxsep=0pt,         % Internal padding between border and text
    colback=Cornsilk1,
    width=\columnwidth,
    % grow to left by=-10pt, 
    % grow to right by=-5pt 
]
\textbf{\ex{Text-Mediated Join Path:}} Let $T_A,T_B\in\mathcal{T}$ be two schematically disjoint tables with no common attributes. A join path is a conceptual link $p=(r_A,S_p,r_B)$ that connects a row $r_A\in T_A$ to a row $r_B\in T_B$ through a set of mediating sentences $S_p\subseteq D$ from a relevant document $D\in\mathcal{D}$. These sentences provide evidence of a latent semantic relationship where no direct relational join condition exists.

\end{tcolorbox}

Our definition of \textbf{Semantic Join Path} introduces a row-to-row linkage mediated by natural language sentences, whereas prior work defined join paths primarily at the table or schema level. In systems such as Metam \cite{GalhotraGF23}, Data Civilizer \cite{MansourDFQTAEIM18}, Aurum \cite{FernandezAKYMS18}, and SemDisc \cite{mohammad2026qualitative}, join paths denote ordered chains of joinable datasets used for augmentation, but these remain purely structural, without textual mediation or record-level grounding. Ver \cite{GongZGF23, DharmawanKGYZGK24} extends this notion to schema-agnostic view discovery with no pre-defined foreign keys. The novelty of our formulated \textbf{tuple-level join path} $(r_A, S_p, r_B)$ lies in its formulation as an explicit fine-grained \textbf{multi-hop transitive bridge} through mediating sentences as evidence of latent relationships. This fundamentally differs from all \textit{prior multi-modal systems}, which target simpler \textbf{one-hop table-text alignments} such as retrieving relevant documents for a table \cite{EltabakhKEA23}.

% None of these approaches explicitly define the fine-grained, \textbf{tuple-level join path} $(r_{A},S,r_{B})$ through mediating sentences as evidence of latent relationships, which is the \textit{core of our contribution}.

\subsection{Problem Statement} \label{sec:problem_statement}

\textbf{\ex{Discovery-Driven Integration:}} Given only a raw multi-modal data lake $\mathcal{L}=(\mathcal{T},\mathcal{D})$, the problem is to infer the missing relational structure for integrating schematically disjoint tables. This requires discovering fine-grained row-sentence alignments that determine the relevant table-document associations $\mathcal{A}\subseteq\mathcal{T}\times\mathcal{D}$ and participating tables $T_A,T_B\in\mathcal{T}$, composing these alignments into row-sentence-row transitive paths $\mathcal{P}$, and inferring a set of latent relationship types $\mathcal{R}$ with a mapping $f:\mathcal{P}\rightarrow\mathcal{R}$ in order to materialize a set of integrated tables:
\[
\mathcal{I} = \{T_{\mathrm{integrated}}^{(R)} \mid R \in \mathcal{R}\}
= T_A \mathrel{{\overset{\mathcal{P}}{\leadsto}}_{\mathcal{R}}} T_B
\]

% \textbf{\ex{Discovery-Driven Integration:}} Given a raw multi-modal data lake $\mathcal{L}=(\mathcal{T},\mathcal{D})$, without a target table pair, table-document links, relationship schema, or analytical query supplied in advance, the problem is to discover the relevant table-document associations $\mathcal{A}\subseteq\mathcal{T}\times\mathcal{D}$ and identify the participating disjoint table pairs $(T_A,T_B)\in\mathcal{T}$. For each discovered table pair, this requires recovering a set of semantic join paths $\mathcal{P}$ and deriving a mapping function $f:\mathcal{P}\rightarrow\mathcal{R}$, where $\mathcal{R}$ is the set of latent relationship types inferred from the discovered paths, in order to materialize a set of integrated tables:
% \[
% \mathcal{I} = \{T_{\mathrm{integrated}}^{(R)} \mid R \in \mathcal{R}\}
% = T_A \mathrel{{\overset{\mathcal{P}}{\leadsto}}_{\mathcal{R}}} T_B
% \]

\begin{table*}[t]
\caption{Comparison of LOKI with State-of-the-Art Data Discovery and Integration Systems.}
\label{tab:sota-related-work}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|llll}
\toprule
\textbf{Category}                                                               & \textbf{Representative Works}                                                        & \textbf{Primary Focus}                                                          & \textbf{Granularity}  & \textbf{Key Limitation (Addressed by LOKI)}                                                                                                 \\ \midrule
\textbf{Semantic Table Discovery}                                               & \begin{tabular}[c]{@{}l@{}}DeepJoin \cite{Dong0NEO23}, OmniMatch \cite{Koutras2025}\\ Snoopy \cite{GuoMHCG25}, FREYJA \cite{MaynouFREYJA24}, \\ KGLids \cite{HelaliMVCHCAH024}, SANTOS \cite{KhatiwadaFSCGMR23} \end{tabular} & Semantic Join                                                                   & Column/Table          & \begin{tabular}[c]{@{}l@{}}Limited to structured signals; fails when \\ the join relationship is hidden in external text.\end{tabular}      \\ \hline
\textbf{Joint Representation}                                                   & \begin{tabular}[c]{@{}l@{}}Termite \cite{FernandezM19}, SEMPROP \cite{FernandezMQEIMO18},\\ TaBERT \cite{YinNYR20}, PNEUMA \cite{BalakaAWGKF25}\end{tabular}           & Embedding Space                                                                 & Schema/Document       & \begin{tabular}[c]{@{}l@{}}Coarse-grained retrieval;\\ lacks explicit row-to-sentence alignment.\end{tabular}                               \\ \hline
\textbf{Multi-Modal Discovery}                                                  & \begin{tabular}[c]{@{}l@{}}CMDL \cite{EltabakhKEA23}, TabSTAR \cite{tabSstar2025},\\ Tri-Encoder \cite{kostic21}, OTTER \cite{HuangZLGJD22}\end{tabular}                   & Table-Text Retrieval                                                            & Table-Document        & \begin{tabular}[c]{@{}l@{}}Relies on pre-existing entity links;\\ fails to discover the semantic relationships.\end{tabular}                  \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Schema/Query-Driven \\Integration\end{tabular}}  & \begin{tabular}[c]{@{}l@{}}ELEET \cite{UrbanB24}, ConnectionLens \cite{AnadiotisBCGHMM22}\\ ThalamusDB \cite{JoT24}, iDataLake \cite{00020F25}\end{tabular}               & Query Execution                                                                 & Query Result          & \begin{tabular}[c]{@{}l@{}}Query-dependent; \\ assumes the user already knows the schema.\end{tabular}                                      \\ \bottomrule
\rowcolor[HTML]{EFEFEF} 
\textbf{\begin{tabular}[c]{@{}l@{}}Discovery-Driven\\ Integration\end{tabular}} & \textbf{LOKI (Ours)}                                                                                                                                                                                                             & \textbf{\begin{tabular}[c]{@{}l@{}}Text-Mediated Join\\Path Discovery\end{tabular}} & \textbf{Row-Sentence} & \multicolumn{1}{c}{\cellcolor[HTML]{EFEFEF}\textbf{—}} \\ \bottomrule
\end{tabular}%
}
\end{table*}


